Single-soft emissions for amplitudes with two colored particles at three loops

We compute the three-loop correction to the universal single-soft emission current for the case of scattering amplitudes with two additional color-charged partons. We present results valid for QCD and $\mathcal{N}=4$ super-symmetric Yang-Mills theory. To achieve our results we develop a new integrand expansion technique for scattering amplitudes in the presence of soft emissions. Furthermore, we obtain contributions from single final-state parton matrix elements to the Higgs boson and Drell-Yan production cross section at next-to-next-to-next-to-next-to leading order (N$^4$LO) in perturbative QCD in the threshold limit.

==> bibliography.tex <==
\begin{thebibliography}{99}
%\cite{Moch:2004pa}
\bibitem{mocht:ns} 
  S.~Moch, J.~A.~M.~Vermaseren and A.~Vogt,
  %``The Three loop splitting functions in QCD: The Nonsinglet case,''
  Nucl.\ Phys.\ B {\bf 688}, 101 (2004)
  [hep-ph/0403192].
  %%CITATION = HEP-PH/0403192;%%
  %689 citations counted in INSPIRE as of 24 Apr 2015
  
  %\cite{Vogt:2004mw}
\bibitem{mocht:si} 
  A.~Vogt, S.~Moch and J.~A.~M.~Vermaseren,
  %``The Three-loop splitting functions in QCD: The Singlet case,''
  Nucl.\ Phys.\ B {\bf 691}, 129 (2004)
  [hep-ph/0404111].
  %%CITATION = HEP-PH/0404111;%%
  %559 citations counted in INSPIRE as of 24 Apr 2015





\end{thebibliography}


